Predictive Sampling: Real-time Behaviour Synthesis with MuJoCo

We introduce MuJoCo MPC (MJPC), an open-source, interactive application and software framework for real-time predictive control, based on MuJoCo physics. MJPC allows the user to easily author and solve complex robotics tasks, and currently supports three shooting-based planners: derivative-based iLQG and Gradient Descent, and a simple derivative-free method we call Predictive Sampling. Predictive Sampling was designed as an elementary baseline, mostly for its pedagogical value, but turned out to be surprisingly competitive with the more established algorithms. This work does not present algorithmic advances, and instead, prioritises performant algorithms, simple code, and accessibility of model-based methods via intuitive and interactive software. MJPC is available at: github.com/deepmind/mujoco_mpc, a video summary can be viewed at: dpmd.ai/mjpc.

==> sections/gui.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\textwidth]{figures/gui.png}%
    \caption{Graphical User Interface. The left tab includes modules for Tasks and the Agent. In the Task module, models are selected from a drop-down menu and the risk value is set; cost weights and residual parameters are specified with interactive sliders. The Agent module provides access to a drop-down menu for planners, settings, and switches that toggle the planner and controller. The right tab includes simulation readings and predictions for the cost, including individual terms, and actions. Live, planner-specific information and various compute time results are shown below. Traces of the current policy and sampled trajectories are visualised and the user can interactively pause or slow down the simulation and apply external forces and moments to the system.}%
    \label{fig:gui}
\end{figure*}


==> sections/macros.tex <==
% macros
\newcommand{\cost}{{c}}
\newcommand{\precost}{{l}}
\newcommand{\state}{{x}}
\newcommand{\nextstate}{{x'}}
\newcommand{\control}{{u}}
\newcommand{\objective}{{J}}
\newcommand{\residual}{{r}}
\newcommand{\app}{{MJPC}}

\newcommand{\plan}{{\mathbf{\Pi}}}

 \newcommand{\yt}[1]{
 {\textcolor{red}{\textbf{[#1 --YT]}}}}



